Virtualizing Intermittent Computing

Intermittent computing requires custom programming models to ensure the correct execution of applications despite power failures. However, existing programming models lead to programs that are hardware-dependent and not reusable. This paper aims at virtualizing intermittent computing to remedy these problems. We introduce PureVM, a virtual machine that abstracts a transiently powered computer, and PureLANG, a continuation-passing-style programming language to develop programs that run on PureVM. This virtualization, for the first time, paves the way for portable and reusable transiently-powered applications.

==> [IEEE Internet of Things Journal] Virtualizing Intermittent Computing/1-introduction.tex <==
\section{Introduction}

\IEEEPARstart{I}{n} the past decade, the progress in energy harvesting circuits and the decrease in power requirements of processing, sensing, and communication hardware promised the potential of freeing the Internet of Things (IoT) devices from their batteries. Recent works demonstrated several microcontroller-based devices that can work without the need for batteries by harvesting energy from ambient sources, such as solar and radiofrequency~\cite{hester2017flicker,yildirim2018safe,nardello2019camaroptera}. Batteryless devices store the harvested ambient energy into a tiny capacitor that powers the microcontroller and peripherals. A batteryless device can compute, sense, and communicate when the energy stored in its capacitor is above an operating threshold. It turns off and loses its volatile state (e.g., the contents of the CPU, peripheral registers, the volatile memory) when the energy level drops below this threshold. The device can turn on only after charging its capacitor again. This phenomenon, i.e., the intermittent execution due to power failures, led to the emergence of a new computing paradigm, the so-called \emph{intermittent computing}~\cite{yildirim2018ink,kortbeek2020TICS}. 

During intermittent execution, batteryless devices use the harvested energy to perform a short burst of computation.  To recover their computation state and progress computation forward after a power failure, they need to save the computation state in non-volatile memory before a power failure. Recent studies proposed programming models for intermittent computing to support these state logging and recovery operations. The proposed programming models provide language constructs (i.e., either \emph{checkpoints}~\cite{kortbeek2020TICS} or \emph{tasks}~\cite{colin2016chain}) to (i) maintain the forward progress of computation and (ii) keep the memory (i.e., computation state) consistent. However, with these models, programmers need to deal with the low-level details of the intermittent execution~\cite{durmaz2019puremem}. In particular, existing models pose the following deficiencies.

\noindpar{Explicit Burst Management.} Programmers need to design their programs as a set of computation bursts that should fit in the capacitor. Thus, they explicitly identify the boundaries of these bursts via checkpoint placement or task decomposition. This situation increases the programming effort considerably.%, making programs \emph{error-prone}, and decreasing the \emph{maintability} and  \emph{readibility} of programs. 

\noindpar{Hardware Dependency.} The active time of a batteryless device depends on its capacitor size and its power consumption, i.e., its hardware configuration~\cite{colin2018reconfigurable}. Programmers might need to identify different burst boundaries to execute their programs on a new device with a different hardware configuration. Therefore, existing intermittent programs are not portable, and in turn, not reusable. 
    
\noindpar{Explicit I/O Management.} Power failures that occur during I/O or interrupt handling might leave the memory in an inconsistent state. With existing models, programmers need to manually ensure the atomic execution of interrupt handlers or I/O operations~\cite{ruppel2019Coati}. This situation increases the programming burden and makes programs error-prone. 

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{pics/purevm.pdf}
    \caption{Using \langname, a continuation-passing-style programming language, and \vmname, whose specification enables the execution of programs written in \langname, programmers do not reason about the intermittent execution and they develop programs portable across several hardware platforms.}
    \label{fig:intro}
\end{figure}

%In this paper, we ask how intermittent computing can be virtualized to abstract the details of intermittent execution and let the programmers focus only on their application logic. In general, we aim to enable the programmers to program intermittently powered devices similar to programming continuously powered systems and develop intermittent programs that are portable across different hardware platforms. To this end,  this paper introduces the following contributions: 
In this paper, we aim at virtualizing intermittent computing to remedy the deficiencies mentioned above. We introduce \vmname virtual machine and its software interface \langname language that abstract away the complicated aspects of intermittent execution. Thanks to \vmname and \langname, programmers focus only on their application logic, forget about power failures as if they are programming continuously powered systems, and develop portable intermittent programs. Shortly, this paper introduces the following contributions:  
\begin{compactenum}
    \item \textbf{\vmname Virtual Machine.} We introduce \vmname, the first \emph{virtual machine} for intermittent systems, which abstracts a transiently powered computer. This abstraction hides the details of intermittent execution and enables platform-independent program development via its implementations targeting different hardware (see Figure~\ref{fig:intro}). %\vmname reduces the intermittent computing to the \emph{continuation}, event, and I/O handling.
    
    %We introduce %the first virtual machine to intermittent computing, named 
    %\vmname that provides a specification for a \emph{virtual machine} to abstract a transiently powered computer. This abstraction enables platform-independent program development via its implementations targeting different hardware (see Figure~\ref{fig:intro}). \vmname reduces the intermittent computing to the \emph{continuation}, atomic event, and I/O handling. %\vmname ensures the progress and correct execution of intermittent programs despite power failures.
    
    \item \textbf{\langname Language.} We introduce \langname, a  \emph{continuation-passing-style} programming language, intended to prevent programmers from reasoning about intermittent execution.  %Programmers develop %\langname programs using objects and functions that operate on these objects. 
    \langname programs are translated into a set of re-composable and atomically-executed \vmname instructions.  
    
\end{compactenum}
To the best of our knowledge, our work proposes the first \emph{virtualization} attempt for intermittent computing. \vmname and \langname create the fundamental building blocks of intermittent computing from scratch that pave the way for portable transiently-powered applications.



%%%%%%%%%%%%%%%%%% BACKUP


%The rest of the paper is organized as follows: In Sect. 2... \geylani{Çağlar diğer bölümlerin içeriklerini birer cümle yazarak burada makalenin geriye kalan kısmını tanıt.}

%This work creates the building-blocks of intermittent computing from scratch. \vmname reduces the intermittent computing to the continuation, atomized event, and atomized peripheral input, which provides static energy consumption easy to reason in compile-time and correct program with I/O. \langname provides artifacts that abstract the programs as re-composable code in an instruction (atomic) level for efficient and platform-independent codes. \sinan{We implemented \vmname in .... and evaluated using.... Our evaluation showed that \vmname is better....}


% Since it does not meet the abstraction needs of transiently powered computers

% The state-of-the-art intermittent systems adopt the tools and abstractions (C language) of continuous powered systems because of their sophistications. However, chekcpointing systems suffer from the dynamic energy consumption, causing inefficiency and platform-dependent code while task-based systems suffer from programmability (reusable, maintainable, readable code) and also platform-dependency.  



%---------------
\iffalse

% some background

With the expansion of the usage areas of IoT applications, the use of battery-powered devices is increasing in places where power transmission is not possible by cable. However, it is necessary to change the batteries of the battery-powered devices from time to time and to dispose of the batteries. 

\IEEEPARstart{T}{he} emerging trend in energy harvesting and low-power microelectronics enabled the microcontroller-based systems that can operate without batteries. 

in energy harvesting circuits and microelectronics have led to a new type of computing systems; namely transiently powered computers (TPCs), that can operate relying on ambient energy only without requiring batteries. As an example, Wireless Identification and Sensing Platform (WISP)~\cite{smith2013wirelessly} is a tiny computer that operates by using the captured energy of radio waves. The captured energy is stored in a small capacitor and if the stored energy is above a threshold, WISP wakes up to sense the environment and perform computation. When the energy in the capacitor is depleted, WISP dies due to a power failure---leading to an intermittent operation. As opposed to continuously-powered computers, TPCs follow a duty cycle composed of charge$\rightarrow$operate$\rightarrow$die phases~\cite{ransford2012mementos}. Since the ambient energy is non-deterministic, TPCs experience frequent power failures which reset the volatile state of the device; e.g. stack, program counter, registers. Therefore, existing programs and libraries designed for continuously-powered computers cannot run on TPCs correctly due to the frequent loss of volatile state---power failures give rise to failed computation and incorrect results. 

% What is the state of the art

In order to preserve progress of computation in TPCs, the researchers proposed inserting checkpoints in the program source at compile time \cite{ransford2012mementos,woude2016ratchet,lucia2015simpler,jayakumar2014quickrecall,mottola2017harvos,balsamo2016hibernus++}, so that the whole volatile state of the processor is saved in non-volatile memory. Upon reboot, the volatile state will be recovered  using the checkpointed information and the computation will be restored from where it left. However, checkpointing introduces considerable store/restore overhead due to the size of the volatile state. This issue motivated researchers to develop task-based programming models for TPCs~\cite{colin2016chain,alpaca,hester2017timely,yildirim2018ink}. In these models, the program source is composed of a collection of restartable tasks, task-based control flow and input/output channels for the data flow among the tasks. Task-based programming environments do not checkpoint the whole volatile state: they execute the current task in the control flow, restart it upon recovery from a power failure, guarantee its atomic completion, and then switch to the next task in the control flow.    

% problem statement
 
However, as compared to the structured programming languages such as C, existing task-based programming models provide limited abstractions and in turn expose several disadvantages. In particular, in current task-based systems (a) control flow statements lead to "spaghetti code", (b) tasks are tightly-coupled with each other since they share global input/output data that decreases their re-usability, (c) tasks do not have signatures and therefore make computation vulnerable to potential bugs and (d) automatic and dynamic memory management is not allowed that leads to a bigger memory footprint. This paper addresses these issues and introduces  a structured task-based programming model for TPCs; namely PureMEM. We list the main contributions of PureMEM to the state-of-the-art as follows: 

\begin{enumerate}

\item Contrary to parameterless tasks and task-based control flow in existing programming models, PureMEM enables signatures for the functions and introduces function composition as a control flow structure in order to \emph{\textbf{eliminate "spaghetti code"}} and to \emph{\textbf{reduce bugs}}. Thanks to continuation-passing style, PureMEM prevents interdependencies caused by the unstructured control and enables \emph{\textbf{re-usability}} of the tasks.
	
\item PureMEM enables manual (dynamic) memory management that allows creation of variables which live longer by providing allocation and deallocation of nonvolatile memory. These variables can be used for data sharing among the tasks---\emph{\textbf{limiting}} the \emph{\textbf{scope}} and \emph{\textbf{lifetime}} of task-shared variables in contrast global scope and lifetime task-shared variables in existing models.  

\item While prior works  \cite{alpaca, colin2016chain, hester2017timely} do not contain any constructs on \emph{\textbf{error handling}}, routines in PureMEM may return and recover errors.
\end{enumerate}

% our contributions 

The rest of the paper is organized as follows: Section 2 includes a brief discussion on TPC and existing programming models for TPC. PureMEM programming model is discussed in Section 3.  Runtime environment of PureMEM is described in Section 4. Use of PureMEM is demonstrated with a case study in Section 5. Section 6 gives the related work and Section 7 concludes the paper.

\subsection{State-of-the-art:} Onceki calismalarda sunlar var. Task-based vs checkpoints. 

\begin{enumerate}
\item Checkpointing tarafinda degiliz. (nedenini yazmak gerek). \item Task-based systemlerin eksiklerinden sirayla bahsedecegiz.
\item \textbf{Lack of mechanisms for structured programming} 
\item PUREMEM aims to bring \textbf{Task-based structured programming} - konferansta yayinladik. 
\item (0) Tasklar parametre alabiliyo
\item (1) Sphagetti Code and Reusability
\item (2) Error handling 
\item (3) Dynamic memory management 
\end{enumerate}

\subsection{Problem Statement:} PUREMEM de yeterli degil - DSL icin baska bir mekanizma gerek. Onun da dahil oldugu tum sistemlerin asagidaki sorunlari var:

\textbf{Deficiencies of the existing systems:} 

None of the existing systems did not propose a DSL for intermittent stytems.
 A DSL brings the following advantages:
 \begin{enumerate}
     \item Platform independence. Thanks to this, platfrom-dependent issues such as code optimization, capacitor size, task-sizes, I/O is abstracted from the programmer.
     \item Event driven programming is easier
     \item PL features like type checking is enabled (for the first time!) that will eliminate bugs, other issues
     \item Code development efforts (bakariz daha sonra)
 \end{enumerate}
 
 \textbf{DSL - Lambda-calculus - Fonmsiyonkel Programlama - Scala} bunlar arasindaki iliskiyi gosterirsek, butunlugu saglamis oluruz. Ya da neden feyz aldik? Diger Task-based calismalarda bunlarin hicbirinden bahsedilmemis. (Unstructured olduklari icin) 

We propose a VM that will execute the code generated by the DSL compiler. These features 
\textbf{PUREMEM vs VM}
\begin{enumerate}
    \item Primitive instruction-like tasks -> VM'e goturuyor
    \item Program VM instructionlarini kullaniyor -> Program tamamiyle HW independent
    \item Prograci da insitruction ekleyebilir (limited degiliz)
    \item VM provoides comple-time optimization for the efficient execution
\end{enumerate}

\begin{enumerate}
\item \emph{Optimized code is decoupled from hardware:} Compiler adjusts the task sizes with regards to the capacitor size of the device. 
\item B-FreeVM provides an event driven programming model which enables sleep mode.
\item B-Free compiler provides a type checking mecahnism with parametric polymorphism, which reduces the bugs.
\item B-FreeVM is also implemented for personal computers, which brings the advantage of testing without micro-controllers.
\item Memory and cache of BFreeVM can be configured and optimized with regards to the application needs. 
\end{enumerate}

\fi


%The building blocks of computer systems have been developed with the assumption of continuous energy. Intermittent computing eliminates continuous energy. However, state-of-the-art intermittent systems use tools (e.g., LLVM compiler and its tools) and languages (e.g., C language) made with the assumption of continuous energy because of their widespread use and level of sophistication. This situation has created some difficulties for systems operating with intermittent energy. State-of-the-art checkpointing systems suffer from dynamic energy consumption due to the C language's call-stack operations, causing inefficiency and platform-dependent code. In contrast, task-based systems suffer from programmability (reusable, maintainable, readable code) and platform-dependency because of poor compiler support.  

%, where the energy stored in the capacitor should be spent to perform a burst of useful tasks and save the systems state in \emph{non-volatile memory} to recover upon a power failure.

%Existing studies presented custom programming models (supported by runtime systems) to bridge the gap between the underlying intermittent execution of the device and the batteryless applications. These programming models provide the necessary programming constructs to maintain the progress of computation and keeping the memory (i.e. volatile state) consistent despite the power failures. Applications developed using these programming models are either: (i) standard C programs paired with \emph{checkpoints}~\cite{ransford2012mementos,woude2016ratchet,lucia2015DINO,maeng2018Chinchilla,kortbeek2020TICS,mottola2017harvos} where the volatile state of the processor (i.e., registers, global data and stack) is stored in non-volatile memory, and upon recovery from a power failure, the computation is continued from the latest saved volatile state, or (ii) \emph{task-based} programs~\cite{alpaca,colin2016chain,yildirim2018ink,ruppel2019Coati,majid2020Coala} which are decomposed into idempotent and atomic tasks that attempt to execute repeatedly until completing uninterrupted. 

%\noindpar{Problem Statement:} Existing programming models for intermittent systems do not obscure the details of the device's intermittent execution and hardware configuration. %, which complicates the program development conceptually.Moreover, their programming constructs are not sufficient to express safe I/O and interrupt driven operations. 

==> [IEEE Internet of Things Journal] Virtualizing Intermittent Computing/2-related.tex <==
\section{Background and Related Work}
\label{sec:background}

Frequent power failures lead to intermittent execution that poses several challenges to developing batteryless applications. We classify these challenges into two classes: computation and I/O related challenges (A1--A3) and programming challenges (B1--B2). We describe them as follows.

\noindpar{A1- Non-termination and Memory Consistency.} Power failures hinder the \emph{forward progress} of the computation, which leads to non-terminating programs~\cite{maeng2018Chinchilla}. Non-termination occurs since the device loses the intermediate results and restarts the computation from scratch upon each reboot. Power failures might also lead to \emph{memory inconsistencies}~\cite{ransford2014nonvolatile}. To give an example, assume that a program is modifying the persistent variable \code{var} (i.e., a variable kept in non-volatile memory) by executing the code block \code{\{vector[var++]=10;\}}. Since the variable \code{var} is updated after it is read, there is a \emph{Write-After-Read  (W.A.R.)} dependency.  If a power failure occurs at this point, the re-execution of this code will increment the variable \code{var} again. Therefore, another element of the \code{vector} will be set to 10 in this case. Due to the W.A.R. dependency, there is a violation of \emph{idempotency} since repeated computation produces different results. To prevent these issues, programmers should divide their programs into a set of idempotent code blocks (e.g., \emph{tasks}~\cite{colin2016chain}) that can execute \emph{atomically} in a power cycle and can be safely restarted despite W.A.R. dependencies. A runtime library (e.g., \cite{alpaca,yildirim2018ink}) is required to persist the program state non-volatile memory, to manage power failures, and to re-execute the code blocks that could not complete in the previous power cycle.

\noindpar{A2- Control-flow Inconsistencies.}  If the control flow depends on external inputs such as sensor readings, power failures might lead to erratic program behavior~\cite{surbatovich2019dependent}. In particular, programmers need to pay special attention to implementing conditional statements that check persistent variables, whose values might be updated during I/O operations. For example, consider the case that a program reads a temperature value (\code{temp = read\_sensor();}) and sets the variable \code{alarm} based on the temperature reading (\code{if(temp > limit) then alarm = true; else tempOk = true;}). If the temperature is less than a pre-defined limit, the variable \code{tempOK} will be set to true. If there is a power failure right after this operation and the program re-executes, the program might read another temperature value higher than the limit. In this case, the program will set the variable \code{alarm} to true. At this point, both of the variables \code{alarm} and \code{tempOK} are true, which is logically incorrect~\cite{surbatovich2019dependent}. %One option is to preserve memory consistency during I/O operations persisting the external input values and control flow before the branch~\cite{alpaca}.

\noindpar{A3- Handling Interrupts.} Interrupts cause dynamic branches, which move the control from the main thread of execution to the interrupt service routine. The main program and interrupt service routines might share the persistent state. If an interrupt service routine leaves the shared persistent variables partially updated due to a power failure, this situation might lead to memory inconsistencies~\cite{ruppel2019Coati}.  

\noindpar{B1- Platform Dependencies.} The execution time of an intermittent program depends on several factors, such as available harvestable energy in the environment, capacitor size (i.e., energy storage capacity), and the energy consumption profile of hardware and software. Intermittent programs need to be modified and restructured regarding these factors to eliminate non-termination and ensure computational progress~\cite{maeng2018Chinchilla}. 

\noindpar{B2- Reuse and Maintaining Difficulties.} Platform and runtime dependencies make implementing reusable intermittent programs difficult~\cite{durmaz2019puremem}. For example, programmers using task-based models need to deal with task decomposition and task-based control flow~\cite{colin2016chain}. Handling these issues is complicated and leads to programs that are difficult to maintain.

\subsection{The State of the Art}

We classify the prior art based on how they addressed the aforementioned challenges.

\noindpar{Checkpoint-based Systems.} %The C language enables structured programming with its direct-style using call-stack for reusable, maintainable, and readable programs. 
Checkpointing runtime environments (e.g.,~\cite{ransford2012mementos,lucia2015DINO,jayakumar2014quickrecall,balsamo2016hibernus++}) persist the registers, global variables, and the call-stack of programs into non-volatile memory via programmer-inserted checkpoints to preserve the forward progress of computation (A1).  In particular, due to the call stack's dynamic nature (i.e., it grows and shrinks dynamically), the programmers need to place checkpoints carefully to eliminate non-termination. In particular, the energy required to execute the instructions between two checkpoints should not exceed the maximum energy stored in the capacitor. Therefore, checkpoint placement is platform-dependent and checkpointed programs are not reusable. There are studies (e.g.,~\cite{woude2016ratchet,mottola2017harvos,kortbeek2020TICS,maeng2020CatNap,maeng2019Samoyed,maeng2018Chinchilla}) that provide compilers to translate C programs into intermittent programs without programmer intervention. However, the C language does not provide abstractions for interrupt handling (A3) and atomic I/O (A2) operations on intermittent systems. The absence of these abstractions might lead to memory inconsistencies and non-termination.

\noindpar{Task-based Systems.} Task-based models (e.g.,~\cite{colin2016chain,alpaca,yildirim2018ink,hester2017mayfly,majid2020Coala,ruppel2019Coati}) require programmers to structure their programs as a collection of idempotent and atomic tasks. They eliminate the need for the call-stack and checkpoints by employing GOTO-style transitions among tasks, i.e., task-based control-flow. However, this is an unstructured programming style that leads to programs that are not reusable and that are prone to bugs~\cite{dijkstra1968letters}. Task-based programming also leads to platform-dependent code since task sizes depend on the capacitor size of the platform. Recent work~\cite{durmaz2019puremem} provides tasks with parameters and continuation-passing~\cite{sussman1998scheme} via closures, which enables reusable code by delivering the control flow in a structured way, similar to function calls. However, it also leads to platform-dependent code because of static task sizes.

\input{table}

\subsection{Our Differences}  

Table \ref{table:runtime_comparison} provides a comparison of our work with the state-of-the-art. We propose an intermittent computing solution composed of a virtual machine (\vmname), a programming language (\langname), and a compiler. We design \vmname to abstract the intermittent execution details and give the programmer a continuously powered view of the target device. This abstraction provides platform-independent code via its multiple compilers for multiple hardware. \langname is the software interface of \vmname. \langname programs are translated into a sequence of \emph{primitive functions}, which are the smallest computation blocks that \vmname executes atomically despite power failures. Thanks to this two-layered abstraction, our work overcomes all mentioned challenges of intermittent computing (i.e., A1--A3 and B1--B2).

==> [IEEE Internet of Things Journal] Virtualizing Intermittent Computing/3-purelang.tex <==
\section{\langname Language}
\label{sec:language}

%\langname is a statically-typed and event-driven programming language. Programmers develop \langname applications via objects and functions that operate on them, and do not reason about intermittent execution. The \langname compiler translates the source program into the \vmname  program that runs correctly despite power failures.

%In \langname, expressions and functions take one \emph{flow-in object}, pass one \emph{flow-out object} to the next expression or function, which is aligned with the \vmname's single-input-single-output architecture. \sinan{As depicted in Fig.~\ref{fig:control_flow} Line 5, \code{apply} primitive function takes the flow-in object \code{a} (which is of parametric type \code{\%a}) and passes a flow-out object of parametric type \code{\%b}. As we explain later, parametric types are used to specify the type later and primitive functions are executed atomically.} This feature enables composable code and structured programming. \langname implements the continuations, i.e.,  program state and the control flow, via anonymous functions\footnote{Anonymous functions have no name. They can be assigned to variables, used as arguments, and invoked later in the functions they are sent to.}. Since the continuations are composed of a function reference and a certain number of object references, the overhead of persisting the continuation is static in contrast to persisting the whole call-stack whose size is dynamic. Since \langname functions always operate on objects, this brings the ability for \vmname to intervene or track the updates on non-volatile object memory, which is described in Section \ref{sec:vm1}, to preserve data consistency between two executions interrupted by a power failure. Functions and expressions update global and local objects and create I/O side-effects (e.g., actuation).
%An event is another type of continuation (i.e., an object and a method to be applied) stored in an event buffer. At any time, the associated \vmname runs an event in the form of continuation (i.e., objects and methods to be applied) in object memory. 

%\langname employs continuation-passing style~\cite{sussman1998scheme} where the program control flow is passed explicitly via \emph{continuations}. Each function (or expression) takes one \emph{flow-in object} in addition to its parameters and passes one \emph{flow-out object} to the next function (or expression) which handles the rest of the computation. Therefore, each continuation contains a reference to a flow-in object,  a set of object references as parameters, and a function reference to be applied. Events are also continuations that are created by interrupt service routines. 

\langname is a statically-typed and event-driven programming language. Programmers develop \langname applications via objects and functions that operate on them, and do not reason about intermittent execution. \langname employs continuation-passing style~\cite{sussman1998scheme} where the program control flow is passed explicitly via \emph{continuations}. Each function (or expression) takes one \emph{flow-in object} in addition to its parameters and passes one \emph{flow-out object} to the next function (or expression) that handles the rest of the computation. Therefore, each continuation contains a reference to a flow-in object,  a set of object references as parameters, and a function reference to be applied. Events are continuations that are created by interrupt handlers. 

\vmname persists continuations in non-volatile memory to ensure forward progress. The overhead of persisting a continuation is static (since it contains only a function reference and a certain number of object references) compared to persisting the call-stack whose size is dynamic in procedural languages. During program execution, \vmname applies the function on the flow-in object by using the information stored in the current continuation. Since \langname functions always operate on objects (kept in non-volatile memory), \vmname can track the updates on these objects to preserve data consistency despite power failures. 

\begin{figure}
	\centering
	\includegraphics[width=0.85\linewidth]{pics/basics.pdf}
	\caption{\langname example primitive and control-flow functions. The control-flow only depends on two primitive functions \textit{apply} and \textit{select} in \langname.}
	\label{fig:control_flow}
\end{figure}

\subsection{\langname Types and Primitive Functions}

\label{sec:io:primitive}

Primitive functions are the high-level instructions, which execute atomically and form the interface between the \langname and \vmname. As an analogy with task-based systems~\cite{colin2016chain,yildirim2018ink,alpaca,ruppel2019Coati,hester2017mayfly,bakar2021rehash}, primitive functions are the atomic tasks that are reusable building blocks. \langname programs are a composition of these atomic blocks. 

\noindpar{Parameteric and Arrow Type.} \langname has built-in object types \code{Int}, \code{Float}, \code{Bool} and \code{Void}, which are reference types that point an address in memory. Moreover, \langname offers \emph{parametric types} that are used to specify the type later. As an example, the \code{select} primitive function (Fig.~\ref{fig:control_flow}, Lines 1--3) returns one of two objects \code{t} or \code{f} of same parametric type \code{\%a} as a flow-out object. The objects referenced by \code{t} and \code{f} can be of any type but same. The primitive function \code{select} makes the decision based on the value of the boolean flow-in object \code{b}. Functions with the parametric type (also known as \emph{parametric polymorphism}) eliminate code duplication. Without parametric polymorphism, \code{select} method needs different implementations for different types. As another example, the  primitive function \code{apply} (Fig.~\ref{fig:control_flow}, Line 5) applies the given function on the flow-in object of parametric type \code{\%a} and  returns a flow-out object of parametric type \code{\%b}. It also takes a function reference \code{func} as a parameter, which takes an object of  parametric type \code{\%a} and returns an object of parametric type \code{\%b}. This is indicated by using \emph{arrow type} decleration depicted as \code{\%a->\%b}. In the body of the primitive function (Fig.~\ref{fig:control_flow}, Line 6), \code{func} is called by passing the flow-in object \code{a}. Note that, \code{func} returns an object of type \code{\%b}, which is compatible with the flow-out object type of  \code{apply}. 

\noindpar{IO Primitives.} \langname introduces IO primitive function functions to eliminate control-flow inconsistencies during I/O operations (A2). \code{IO} metadata (e.g., see \code{getTemp} function in Fig.~\ref{fig:control_flow}, Line 9) helps the \langname compiler to handle these operations differently. The compiler splits \langname code blocks with IO primitives into three sections: pre-IO primitive, IO primitive itself, and post-IO primitive. After each section executes, \vmname takes control to persist computational state, which ensures the atomic execution of the IO primitive. 

\noindpar{Type Checking.} Arrow and parametric type declarations help the \langname compiler for type inference and type checking. While decomposing the program into its primitive functions, the \langname compiler performs type checking by using input and output type metadata to eliminate (B2)-type bugs. The compiler also infers the variable types automatically when the programmer does not declare them explicitly. 

\noindpar{Resolving W.A.R. Dependencies.} Primitive functions also specify a meta-data concerning write operations on objects. As an example, the \textit{write} in the definition of \code{getTemp} function tells the compiler that this function modifies the flow-in object \code{x}. While decomposing the program into its primitive functions,  the compiler can resolve W.A.R. dependencies using this metadata. This situation helps \vmname to execute the intermittent program correctly by preserving the memory consistency (to ensure A1). Considering the target \vmname implementation, \langname compiler instruments the bodies of the functions by inserting the necessary undo logging or redo logging code explained in Section~\ref{sec:vm}.

%\subsection{\langname Type System}

%Two basic types of \langname are primitive type and object type. A \emph{primitive type} is a value type. Built-in primitive types are \code{int}, \code{float}, \code{bool} and \code{void} whose size are dependent on the hardware architecture. An \emph{object type} is a reference type. Built-in object types are \code{Int}, \code{Float}, \code{Bool} and \code{Void}. As an example, the type \code{Int} is similar to the type \code{int*} (pointer to int) in C. It refers a memory area in which \code{int} value resides. 


%\noindpar{Parametric Type.} They are used to specify the type of the function parameters later. As presented in Fig.~\ref{fig:control_flow} (Lines 1--3), the primitive function \code{select} returns one of two objects \code{t} or \code{f} of the same parametric type \code{\%a}. Therefore, the objects referenced by \code{t} and \code{f} can be of any type but same. \code{select} makes the decision based on the value of the boolean input object \code{b}, which is the reference of the object to be processed in the method. Functions with the parametric type (also known as parametric polymorphism) reduce duplicate code. Without parametric polymorphism, \code{select} method needs different implementations for different types.  

%\noindpar{Arrow Type and Type Checking.} The primitive function \code{apply} (Lines 5--7 of Fig.~\ref{fig:control_flow}) takes an input object \code{a} of parametric type \code{\%a} and an anonymous function \code{f} of \emph{arrow type} \code{\%a->\%b}. The arrow type notation indicates that the \code{f} has an input object of parametric type \code{\%a} and returns an object of parametric type \code{\%b}. The function \code{apply} applies the anonymous function \code{f} to the object \code{a} and returns an output object of type \code{\%b}. In other words, it invokes \vmname to execute the operation \code{a.f()}. Arrow types help the \langname compiler for type inference and type checking, which eliminates the bugs related to types (B2). 



%\begin{figure}
%	\centering
%	\includegraphics[width=0.85\linewidth]{pics/primitives.pdf} 
%	\caption{Primitive function implementations in \langname.}
%	\label{fig:io_primitives}
%\end{figure}

%\subsection{\langname Primitive Functions } 

%\label{sec:io:primitive}

%The interface between the instruction on a generic (or particular) hardware and \langname is the primitive function definition. \vmname guarantees the atomic execution of the primitive functions. Primitive functions specify the meta-data concerning read-write memory operations and I/O operations. \langname and the compiler only consider the signature and the metadata of the primitive functions. The signature of the function is used for the type checking to eliminate bugs (B2). Metadata, such as \textit{read, write} in the definition of  \code{add} primitive function in Fig.\ref{fig:io_primitives}, helps compiler to manage W.A.R. dependencies (A1) and ensure \vmname to execute the intermittent program correctly by preserving its memory consistency. Primitive functions need explicit output type declaration. Using the metadata about input and output type of primitive functions and decomposing the program into its primitive functions, the compiler confirms the correctness of expressions and functions in terms of types. It also infers the types when the programmer does not declare the types of variables and functions. Figure~\ref{fig:io_primitives} presents an IO primitive function. \textit{IO} metadata helps to prevent control-flow inconsistencies. \langname compiler splits \langname code blocks with IO primitives into three sections: pre-IO primitive, IO primitive itself, and post-IO primitive. When a section is executed, \vmname takes control to persist computational state. Therefore, the atomic execution of the IO primitive is ensured and (A2) is eliminated. 

\subsection{\langname Statements and Control Flow}

Since \langname employs structured programming, complex expressions are formed by composing other expressions (and primitive functions). The dot operator (\code{.}) enables expression composition as long as the output type of sub-expression is compatible with the input type of the following sub-expression. The last statement in a function body determines the output object that should be compatible with the output type of the function. Thanks to the continuation-passing style of the language, all statements forming the complex behavior of a function execute in order. Therefore, there is no need for the \vmname to check branches and early exits.

\noindpar{Control Flow.} In \langname,  every function related to the control flow is a composition of \code{select} and \code{apply} primitive functions. For example, \code{ifElse} function (Fig.~\ref{fig:control_flow}, Lines 14--16) enables a conditional branch by invoking the \code{apply} and \code{select} primitive functions in order. The first parameter \code{s} is a function that takes an object of parametric type \code{\%a} and returns a boolean object. Firstly, the function \code{s} is applied on the flow-in object \code{p}, which pipes a boolean object (i.e., \code{p.apply(s)} in Line 11 which returns boolean). Then, the returned object becomes a flow-in object for the \code{select} primitive, which returns one of the functions from \code{t} and \code{f} by considering the flow-in boolean object. The returned function object is assigned to variable \code{func}. Then, \code{func} is applied to the flow-in object \code{p}, and an object of \code{\%b}  type is returned (Line 12). 

%In \langname, expressions can be composed to form complex expressions by using "." operator, as long as the output type of sub-expression is compatible with the input type of the following sub-expression. Function body contains sequential statements for composing behavior over an object type. The last expression statement in the body determines the output object and the output type of the function. In other words, there is no return keyword in \langname and consequently no early exit in the functions. This also means that all statements belonging to a function are executed once the execution of the function is started, which enables \vmname to execute the statements of a function in separate execution windows without checking branches and subsequently early exits.

%The primitive functions \code{select} and \code{apply} are the only functions enabling the control flow in a program. Every function (method) related to the control flow is a composition of these primitive functions. For example, the method \code{ifElse} (Fig.~\ref{fig:control_flow} Lines 14--16) is defined for any type (i.e., using parametric types) to enable branching invoking the \code{select} and \code{apply} functions one and after. The first parameter \code{s} is an anonymous function that takes an object of parametric type \code{\%a} and returns a boolean object. Other parameters are two different anonymous functions whose input and output types are of the same type. The first function application (Line 11) pipes a boolean object (i.e., \code{p.apply(s)} operation which returns boolean). The method \code{select} returns one of the anonymous functions from \code{t} and \code{f} considering the boolean object. The anonymous function in the flow assigned to variable \code{func}. An object of \code{\%b}  type is returned after applying the anonymous function in \code{func} (Line 12). See the usages of \code{ifElse} method (Line 11-16) and anonymous functions (Line 20,21) in Fig.\ref{fig:event_handling_configuration}. Similarly, \code{while} function for iterations is implemented using only \code{apply} and \code{select} \caglar{with the signature \code{(a:\%a)while(s:\%a->Bool, f:\%a->\%a)}}.

%Global variables, local variables, and arguments of functions are assigned to an object or a literal/constant value. The global objects are allocated when the program begins, and they are never deallocated.  In automatic storage duration, the storage for the object is allocated at the beginning and deallocated at the end of the function. 

%In \langname, when a variable is assigned to an object, it is not allowed to re-assign it to a new object. The reason is that the \langname compiler can decompose functions into smaller functions and the \vmname persist the continuations with these sub-functions and objects created at runtime. If the pointer points to a different address, then persisted continuations may refer to invalid objects, which cause dangling pointers. 

\begin{figure}
	\centering
	\includegraphics[width=0.95\linewidth]{pics/application.pdf} 
	\caption{Sample monitoring application in \langname. Application code contains all semantics of the computation, \vmname settings defining the events of the program and platform specific attributes. Interrupt code is for receiving the values from environment (e.g., sensors).
	}
	\label{fig:event_handling_configuration}
\end{figure}

%\subsection{\langname Compiler}
%\label{sec:compiler}

%We implemented different \langname compilers using Xtext \cite{eysholdt2010xtext} framework (integrated to Eclipse IDE environment). These compilers target different virtual machine implementations. In general, a \langname compiler requires an application setting file (shown in Fig.\ref{fig:event_handling_configuration}), which contains properties such as the event handler list, the hardware platform, the name of the \vmname implementation, some parameters specific to \vmname (such as non-volatile memory size, the size of the event queue), and optimization parameters (specif to \vmname implementations). Compilers produce C code from the given \langname program. The generated code includes a C file and a header file. In addition to the application code, the produced C file also includes the \vmname  implementation and the \code{addEventQ} function that is the interface with the hardware platform. Compilers wrap the bodies of primitive functions (indicated by the green in Fig.~ \ref{fig:control_flow}) with code that will eliminate memory consistency problems. This extra code can change according to the design of \vmname. For example, the compiled code of the function in Fig.\ref{fig:io_primitives} will be \code{float* getTemp(float* x)\{ undoLog(x,sizeof(float));floatGetTemp(x);\}} in \implI implementation (see Section \ref{sec:vm1}).

\subsection{Putting Things Together: A Sample Sensing Application}

%Figure~\ref{fig:event_handling_configuration} presents an event-driven air conditioning application, which includes three types of code blocks: (1) \vmname settings which define the events and their handlers, (2) \langname code which contains the objects, methods, and globals for processing the events and preserving the state of the computing, and (3) interrupt handlers that trigger \vmname by calling \code{addEventQ} method to insert the events received from the environment. \vmname processes these events and calls methods serving as event handlers (such as \code{control} method). %This kind of loosely coupled architecture helps to platform-independent (B1), reusable (B2) code, and efficient sensor applications using interrupts (A3). 

%\langname compiler (implemented using Xtext~\cite{eysholdt2010xtext}) produces C code from the given \langname program. The generated code includes a single C source file and its header, which also contain the implementation of the target \vmname.  In general, a \langname compiler requires an application setting file, which mainly contains the list of event handlers, the name of the target hardware platform, and some specific parameters of the selected \vmname implementation (such as non-volatile memory size, the size of the event queue). 

%The first three event handlers, boot, reboot, and sleep, are mandatory. The boot event occurs the first time the computer boots after being deployed. The reboot event occurs after recovery from a power failure. Since reboot leads to losing all volatile state of the computer, the reboot handler is the function to store the register settings of the microcontroller such as clocks, timers, and LEDs. \vmname fires the sleep event when there is no event to be processed to put the processor in a low power mode to save energy. The \code{control} event handler in the figure handles the events generated from the interrupt service routine. The \code{buttonPress} function includes IO primitive function \code{getTemp}. PureVM atomically saves the measurement in object memory and then calls the \code{control} function in a separate operation window. This approach prevents the cooler and the heater from turning on at the same time. Therefore, the control-flow inconsistency (A2) is prevented without the intervention of the programmer.

%\caglar{Two properties of anonymous functions are of value to intermittent computing. 1) they can access the variables of the environment in which they were created (i.e. the global variables and the variables of the functions in which they were created) 2) anonymous functions themselves can be assigned to a variable, so they can be sent to other functions and run there. With these two features, the computation state and a set of operations can be stored in memory in a data structure. Operations on state can be split into chunks (i.e. bursts) and run repeatedly and idem-potently.} \caglar{Buradan da fig.4 line 20 21'e referans verilebilir.}

Figure~\ref{fig:event_handling_configuration} presents an event-driven air monitoring application, which includes an application source code and a configuration file. \langname compiler (implemented using Xtext~\cite{eysholdt2010xtext}) produces C code from the given \langname program. The generated code includes a single C source file and its header. The source file also contains the implementation of the target \vmname.  The \langname compiler requires a configuration file, which mainly contains the list of event handlers, the name of the target hardware platform, and some specific parameters of the selected \vmname implementation (such as non-volatile memory size, the size of the event queue). 

The application code contains the objects, methods, and interrupt handlers. The event handlers  \code{boot}, \code{reboot}, and \code{sleep} (which is not shown in the figure), are mandatory. The \code{boot} event occurs the first time the computer boots after being deployed. The \code{reboot} event occurs after recovery from a power failure, which triggers the reboot handler that restores the state of the computation. \vmname triggers the \code{sleep} handler when there is no event to be processed, which puts the processor in a low power mode to save energy. The timer interrupt handler (Lines 19--21) adds an event to the event queue of \vmname by calling \code{addEventQ} method with the sensed temperature value (via \code{readTemp}) and the corresponding event handler (which is \code{control} in this case) as parameters. \vmname processes this event by calling the \code{control} event handler (Lines 9--11), which processes the events generated from the timer interrupt service routine. Inside this routine, the heater is turned on or off based on the received temperature value (Line 10). 


==> [IEEE Internet of Things Journal] Virtualizing Intermittent Computing/4-purevm.tex <==
%\begin{figure}
%	\centering
%	\includegraphics[width=0.9\linewidth]{pics/rewinding.pdf} %,height=13cm width=0.7\columnwidth
%	\caption{The \vmname (\implI implementation) memory layout.}
%	\label{fig:rewinding}
%\end{figure}

\begin{figure*}
	\centering
	\includegraphics[width=\linewidth]{pics/rewinding_in_action.pdf} %,height=13cm width=0.7\columnwidth
	\caption{The steps taken by \implI to execute  the \code{control} event described in Fig. \ref{fig:event_handling_configuration}. In the lower right corner of the figure, a part of the compiler generated code is presented. The compiler splits the \code{control} method into primitive functions and then recomposes into its basic blocks.}
	\label{fig:rewinding-in-action}
\end{figure*}

\section{\vmname Intermittent Virtual Machine}
\label{sec:vm}

%\vmname is a single-input/single-output system composed of an event queue, a non-volatile object memory, and a continuation executed in volatile memory by a \emph{runtime engine} (see Fig. \ref{fig:rewinding-in-action}).  It specifies a primary runtime environment for event-driven intermittent programming. \vmname specification enables running the \langname programs on multiple hardware and secondary runtime environments with different configurations and objectives.

%\vmname consumes the events generated by interrupt routines. \vmname creates a continuation in \emph{object memory} from the event at the head of the queue.  As mentioned,  continuation represents the control state of the computer program, and it consists of a set of objects and methods to be applied. Running a continuation may create/return another continuation. \vmname runs the continuations until there is no returned continuation. Running the program might produce outputs via I/O instructions. When there is no event to consume in the queue, \vmname sleeps until an interrupt generates an event. 

%State of computation is composed of the events in the queue, the continuation of running event, objects, and register settings of the computer. This information, except event queue, is stored in object memory to preserve forward computation progress in case of power failures. Before calling the following method (i.e., running the subsequent continuation), \vmname can decide to persist the state in object memory (maintained in non-volatile memory) in order not to lose the intermediate results in case of power failures. \vmname maintains the integrity of object memory by resolving W.A.R. dependencies by considering the metadata of the primitive instructions.

%\vmname specifies the artifacts (event buffer, object memory, runtime engine, and running program) and their relationships in a highly abstract way. Event buffer can be implemented as a regular first-in-first-out (FIFO) queue or a priority queue as long as the system's single-input behavior, whose events created by preempted interrupts, is not violated. Although the object memory should keep the control state as a continuation, there is no limitation as storing the continuation in a stack data structure or a heap with garbage collection. Different design choices can lead to different \vmname implementations. In the following section, we describe \implI that is the defacto \vmname implementation.

\vmname is a single-input/single-output system that specifies a runtime environment for event-driven intermittent programming. \langname programs execute, without any modification, on different hardware and runtime environments conforming \vmname specification.

\vmname specification comprises an event queue, a non-volatile object memory, and a continuation executed by its runtime engine. \vmname pushes the events generated by the interrupt service routines to the event queue. \vmname removes the event at the head of the event queue and creates a continuation in object memory using that event.  As mentioned,  continuation represents the control state of the computer program, and it consists of a set of objects and methods to be applied. Running a continuation may create/return another continuation. \vmname runs the continuations until there is no returned continuation. When there is no event to consume in the queue, \vmname sleeps until an interrupt generates an event. 

\vmname state (which represents the computational state) is composed of the events in the queue, the continuation of the running event, and the global objects. The object memory region in non-volatile memory maintains the global objects and the running continuation.  Before calling the next function (i.e., running the subsequent continuation), \vmname can decide to persist the state in object memory to preserve forward computation and not to lose the intermediate results in case of power 
failures.

\vmname specifies the artifacts (event buffer, object memory, runtime engine, and running program) and their relationships abstractly. For example, the event buffer can be implemented as a regular first-in-first-out (FIFO) queue or a priority queue, as long as the system's single-input behavior is not violated. Different design choices can lead to different \vmname implementations. In the following section, we describe \implI, which is our main \vmname implementation. 

\subsection{\implI: An Undo-Logging \vmname}
\label{sec:vm1}

\implI stores the execution context in the continuation stack and keeps the object memory consistent across power failures via the undo-logging mechanism. Events in the event queue, global objects, and continuation stack in the object memory represent the computational state. The metadata about the continuation stack is stored in the \emph{runtime data} region of the object memory. 

%\implI provides a queue for event buffering, which holds the event objects, and the methods that need to be applied to these objects (\emph{Event Queue} in Fig.~\ref{fig:rewinding-in-action}). \implI runtime engine stores the continuations in a stack in object memory (\emph{Continuation Stack} in Fig.~\ref{fig:rewinding-in-action}). The runtime engine starts event execution by copying the event object (event-data) and event-method (event-handler) to the continuation stack.  
%Since each event contains an object and each method returns an object, there is always an active object in the process. The runtime engine keeps the active object (i.e., flow object) in object memory (\emph{flow-object} in Fig.~\ref{fig:rewinding-in-action}). \implI reduces the event handling to a single-producer-single-consumer problem which eliminates the race conditions on the event buffer. During execution, the runtime engine pops a method from the continuation stack and runs this method on the flow object. Control passes to the method, and the method makes changes on the objects. Since these changes are done only by calling primitive functions, the undo-log mechanism is activated when making changes to preserve memory consistency. 

%The object memory is divided into blocks called pages---the programmer, for efficiency, may configure the page sizes of the object memory. Every primitive function that modifies objects calls the runtime engine's log function before updating the object. The log function copies the original page to undo-log memory before any update on a page. When \implI reboots after a power failure, it copies all the logged pages (including the pages of runtime data) into their corresponding pages in the object memory and then runs the program. This mechanism ensures the consistency of the object memory by eliminating partial modifications. 


%The method being executed can push other methods to the continuation stack. The method execution finally returns an object and gives the control back to the runtime engine. The runtime engine saves the returned object as a flow object. The runtime atomically clears the undo-log memory as the last operation. In this way, the runtime keeps memory consistent and guarantees the forward progress of the program. Moreover, the runtime engine does not specially treat IO operations.  The compiler splits the program from where the IO primitive functions are called, as described in Section \ref{sec:io:primitive}. 

\noindpar{Event Handling.} \implI provides a queue for event buffering, which holds the event objects and the methods that need to be applied to these objects (\emph{Event Queue} in Fig.~\ref{fig:rewinding-in-action}). \implI runtime engine stores the continuations in a stack in object memory (\emph{Continuation Stack} in Fig.~\ref{fig:rewinding-in-action}). The runtime engine starts event execution by copying the event object (event-data) and event-method (event-handler) to the continuation stack. It is worth mentioning that \implI reduces the event handling to a single-producer-single-consumer problem which eliminates the race conditions on the event buffer. During execution, the runtime engine pops a method from the continuation stack and runs this method on the flow object. Control passes to the method, which can modify the objects. 

\noindpar{Undo-Log and Memory Consistency.} The undo-log mechanism is activated when modifying objects to preserve memory consistency. The modifications on the objects are done only by calling primitive functions. Every primitive function calls the runtime engine's log function before modifying an object. The object memory comprises blocks called pages. The programmer, for efficiency, may configure the page sizes of the object memory.  The log function copies the original page to undo-log memory before any modification on that page. When \implI reboots after a power failure, it copies all the logged pages (including the pages of runtime data) into their corresponding pages in the object memory and continues the program. This mechanism ensures the consistency of the object memory by eliminating partial modifications.  

\noindpar{Forward Progress and Execution Flow.} The method being executed can push other methods to the continuation stack. The method execution finally returns an object and gives the control back to the runtime engine. The runtime engine saves the returned object as a flow object. The runtime atomically clears the undo-log memory as the last operation. In this way, the runtime keeps memory consistent and guarantees the forward progress of the program. 

\noindpar{I/O Handling.} The \langname compiler already splits the program code blocks with I/O primitive functions into three sections, as described in Section \ref{sec:io:primitive}. This strategy already ensures the atomic execution of I/O operations. Therefore, the \implI runtime engine does not treat I/O operations in a specific way.  

\noindpar{\implI Compiler Optimizations.} We implemented two compiler optimizations for \implI: (i) executing several primitive functions as a block, and (ii) some loop optimizations to reduce \vmname overheads such as repetitive undo logging (i.e., page copy) operations. Programmers can modify \vmname application configuration file to enable optimizations. 

\subsubsection{An Example \implI Execution.} 
Fig. \ref{fig:rewinding-in-action} shows how \implI handles the \code{control} event described in Fig. \ref{fig:event_handling_configuration}. In the first step, the interrupt service routine adds the address of the control method to the event queue along with the sensed temperature value (which is a floating-point value of 22.0). In the second step, the VM copies the event from the event queue to the object memory (depicted as \code{control} and \code{22.0} in the continuation stack). In the lower right corner of Fig. \ref{fig:rewinding-in-action}, a part of the compiler-generated code is presented. The compiler splits the \code{control} method into primitive functions and then recomposes into its basic blocks.  As can be seen from the figure, the recomposed version of the \code{ifElse} method (Line 10 in Fig. \ref{fig:event_handling_configuration}) is fragmented into two continuations that represent \code{apply} and \code{select} primitives. In the third step, the VM removes the first method from the continuation stack  (\code{control} function in the lower right corner of Fig. \ref{fig:rewinding-in-action}) and runs it.  Since this process changes the runtime data and the stack of the non-volatile memory, it copies the pages to undo memory before any update. The fourth step in the figure shows that the computer restarts after a power failure. In the fifth step, the VM calls the undo function because it detects that the undo memory is not empty. It brings the non-volatile object memory to the last consistent state. Then, in step 6, the method on the stack runs, as described in step three. In the seventh step, the undo memory is cleared by committing it. Forward progress of the computation is ensured by executing the operations  \code{vm\_consume}, \code{vm\_commit} and \code{undo} atomically. In the next steps (not shown in the figure), the remaining methods in the continuation stack execute. They pass the returned flow objects to the next methods till the continuation stack becomes empty.

\subsection{Other \vmname Implementations}

We also implemented two different \vmname versions, named \implII and \implIII. \implII does not contain an undo log memory and requires hardware support to capture an interrupt when the voltage value on the capacitor crosses the lower-threshold voltage. This interrupt persists the computational state in non-volatile memory and puts the runtime into sleep mode to stop computation. This strategy prevents memory inconsistencies without the need for an undo-log. \implII's overhead is lower than \implI's since \implII does not include page copy operations between log memory and object memory. We implemented \implIII to test any \langname program on a personal computer with continuous power. This implementation allows us to test the correctness of the program logic without loading the code on a microcontroller. 

% Another disadvantage is the correct determination of the lower and upper threshold values. When determining the lower threshold, it is necessary to detect enough energy to complete a \computingloop, the worst-case scenario. If the lower threshold is exceeded and the power is cut before the next runtime cycle, W.A.R. dependency conditions will occur. It can be challenging to determine the lower threshold value for each hardware configuration accurately.


==> [IEEE Internet of Things Journal] Virtualizing Intermittent Computing/5-evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

We evaluated our \vmname implementations considering three compute-intensive applications Cuckoo Filter (CF), Activity Recognition (AR), and  Bit Count (BC). These applications are used as the de facto benchmarks by most of the earlier studies on intermittently powered devices (\cite{kortbeek2020TICS,alpaca,colin2016chain,yildirim2018ink}). CF stores and reads an input data stream using a cuckoo filter with 128 entries and searches the inserted values. AR classifies accelerometer data, computing the mean and standard deviation of a window of accelerometer readings to train a nearest-neighbor model to detect different movements. We used a window size of three and read 128 samples from each class (shaking or stationary) in the training phase. BC counts the number of 1s in a bitstream with seven different methods that are executed 100 times each.

We compiled these applications using the \implI and \implII compilers and executed them on the MSP430FR5994 evaluation board \cite{msp430fr5904}. To power MSP430 evaluation boards intermittently, we used Powercast TX91501-3W transmitter \cite{powercast}, which emits radio frequency (RF) signals at 915 MHz center frequency. P2110- EVB receiver, connected to our MSP430FR5994 evaluation board, harvests energy from these RF signals. We placed the P2110- EVB receiver at a distance of 60cm from the RF transmitter.

\subsection{Execution Time Overhead}
We evaluated the performance of \vmname implementations of the benchmarks on harvested energy and continuous power by considering their execution times. For comparison, we used their InK \cite{yildirim2018ink} implementations since InK is one of the de facto task-based systems for intermittent computing. We directly used InK-based implementations of the benchmarks (CF, AR, and BC) from the InK repository\cite{tudssl_2019}. Since the tasks have fixed sizes in InK, they may exceed the energy buffer of the device, or they may perform inefficiently due to frequent task transitions (causing redo logging of all shared variables to preserve memory consistency). To re-calibrate the size of the tasks, the programmer must recompose all tasks for the new device. This way of programming limits the code portability. 


\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{pics/eval_continuous.pdf} 
	\caption{Normalized execution times of AR, CF and BC benchmarks with InK, \implI and \implII under continuous power.}
	\label{fig:execution_time_1}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{pics/eval_intermittent.pdf} 
	\caption{Normalized execution times of AR, CF and BC benchmarks with InK, \implI and \implII under RF energy harvesting scenario.}
	\label{fig:execution_time_2}
\end{figure}

Fig.~\ref{fig:execution_time_1} and Fig.~\ref{fig:execution_time_2} show the normalized execution times of the benchmarks with InK and \vmname (\implI, \implI optimized, \implII, \implII optimized) on continuous power and intermittent execution on RF-power. The compiled code of \implI and \implII can run on the devices with a minimal energy buffer because the compiler recomposes primitive functions regarding basic blocks. Recomposing the code into its basic blocks leads to small continuations and consequently more (continuation) stack operations in \implI and \implII, and more undo logging operations in \implI. %The continuations based on basic blocks are not efficient. 
Optimized versions of applications are composed of continuations with more operations. Therefore, these applications run more efficiently compared to InK apps. We applied the loop optimizations to all loops and branch optimizations to some branch method invocations in these applications. 

\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{pics/eval_useful_rew.pdf} 
	\caption{RewindingVM overhead, split per operation.}
	\label{fig:rew_portions}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{pics/eval_useful_jit.pdf} 
	\caption{JustInTimeVM overhead, split per operation.}
	\label{fig:jit_portions}
\end{figure}


\subsection{\vmname Point-to-Point overheads}

Fig.~\ref{fig:rew_portions} and Fig~\ref{fig:jit_portions} show the useful work and overheads (i.e., undo-logging and stack operations) of corresponding runtimes on continuous power. \implI and \implII uses a stack to run the continuations. When there is more branching in the program, the continuation stack operation creates more overhead because \implI and \implII run the basic blocks in one cycle, which means every branch needs continuation stack operation. In BC, the overhead of stack manipulation is higher due to many branch operations, which also causes the worst performance compared to other benchmarks. On the other hand, loop optimizations in BC had the most impact on the performance compared to other benchmarks, increasing the performance by a factor of 10.

%Any W or W.A.R. operation on a page triggers the undo-logging mechanism. Before any update on the page, the page is logged if it has not been logged before. Search and page copy operations are the two main overheads of logging. The runtime engine takes advantage of the spatial locality and temporal locality of the objects in use, thanks to its continuation stack and automatically allocated storage in the stack. Since the log memory size is small for the benchmarks, we chose a sequential page search in the log memory. Page size affects the undo logging performance. The virtual machine configuration file of \implI and \implII contains a page size setting. The page size of 32 and 64 bytes gave the best performance in these applications.

Before modifying a page that has not been logged before, the undo-logging mechanism is triggered, which introduces page search and page copy overheads. Since the log memory size is small for the benchmarks, we chose a sequential page search in the log memory. Apparently, the page size affects the undo logging performance. The virtual machine configuration file of \implI and \implII contains a page size setting. The page size of 32 and 64 bytes gave the best performance in these applications.

\begin{table}
\centering
\caption{Memory consumption for three benchmark applications written in InK and \vmname.}
	\label{table:memory_comparison}
\begin{tabular}{ccccccc}
\toprule
  \textbf{App.}& \textbf{Memory(B)}& \textbf{InK} & \textbf{Rew.} & \textbf{Rew.Opt.} & \textbf{JIT} & \textbf{JIT.Opt.}\\
\toprule
\multirow{2}{1em}{AR} & .text & 3822 & 8624  & 6810  & 7950  & 6136\\
                      & .data & 4980 & 694   & 694   &  420  & 420\\
\multirow{2}{1em}{BC} & .text & 3518 & 11258 & 9928  & 10714 & 9378\\
                      & .data & 4980 & 882   & 882   & 676   & 548\\
\multirow{2}{1em}{CF} & .text & 2708 & 11980 & 10014 & 11302 & 9350\\
                      & .data & 5213 & 886   & 694   & 804   & 420\\
\bottomrule
\end{tabular}
\end{table}

\subsection{\vmname Memory overheads}
Table \ref{table:memory_comparison} shows the memory overheads of InK and \vmname implementations. Since primitive functions are translated into C codes, PureVM programs have larger code sizes than InK programs. InK uses global shared variables for communication among functions, and hence it has larger data memory than \vmname. The programmer configures data memory of \implI and \implII via the configuration file. The stack size required by virtual machines contributes to their data memory requirements.  The code size increase is the cost which \vmname implementations pay for their performance and platform independence. However, overall results show that the memory requirement of \vmname is comparable with InK's memory requirement.

\begin{figure}
	\centering
	\includegraphics[width=0.6\columnwidth]{pics/eval_photo.pdf} %,height=7cm
	\caption{Our testbed deployment used to evaluate our HVAC application.}
	\label{fig:AirConditioner}
\end{figure}


\subsection{Case Study: Heating, ventilation, and air conditioning  (HVAC) controller}
As a case study to demonstrate the applicability of \vmname, we developed an air condition controller for home automation (Figure ~\ref{fig:AirConditioner}). The goal is to get the room temperature frequently enough and send a message to home automation to keep the room temperature in the ideal temperature range. The application uses the \vmname event mechanism to reduce energy consumption as much as possible: after controlling the room temperature, the application switches to sleep mode. A reboot from a power failure or a timer interrupt (with 30-second intervals) triggers the program, which estimates the room temperature using an analog-digital converter configured to the internal temperature sensor of the microcontroller. If the room temperature is not ideal, the application starts asynchronous communication via Nordic nRF52832 \cite{nRF52832} (which supports BLE) using interrupts over the serial peripheral interface. We ran this application for 3 hours. We observed that the temperature of the environment was measured 294 times, and 22 BLE advertisement messages were sent to the HVAC system. During the entire run, there were 18 power failures and recovery.

==> [IEEE Internet of Things Journal] Virtualizing Intermittent Computing/6-conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conc}

In this work, we introduced a new virtual machine (\vmname) that abstracts a transiently powered computer and a new continuation-passing-style programming language (\langname) used to develop programs that run on \vmname. This two-layer structure provided a loosely coupled architecture that facilitates the development of platform-independent and reusable event-driven sensor applications. We believe that this is a significant attempt for virtualizing intermittent computing.

As follow-up work, we plan to add new language constructs to \langname to handle the expiration of sensor readings. Due to long charging times after power failures, sensed data might lose its validity. In this case, the sensor value becomes useless and can be discarded. While such a requirement is absent in continuous computing, it exists in intermittent computing~\cite{kortbeek2020TICS,hester2017mayfly}. We also plan to port \vmname to different ultra-low-power micro-controllers and introduce more sophisticated compiler optimizations. As of now, \vmname does not implement any task scheduling mechanism. We leave integrating scheduling mechanisms, e.g., real-time scheduling of tasks ~\cite{karimi2021real,maeng2020CatNap}, to \vmname as future work. 

 

==> [IEEE Internet of Things Journal] Virtualizing Intermittent Computing/table.tex <==
\begin{table}
%\renewcommand{\arraystretch}{0.9}
\caption{The state of the art runtimes and mentioned challenges.}
\label{table:runtime_comparison}
\centering
\begin{tabular}{>{\centering}m{0.21\textwidth}
			>{\centering}m{0.07\textwidth}
			>{\centering}m{0.009\textwidth}
			>{\centering}m{0.009\textwidth}
			>{\centering}m{0.009\textwidth}
			>{\centering}m{0.009\textwidth}
			m{0.01\textwidth}<{\centering}}
\toprule
  \textbf{Runtime} & \textbf{Type} & \textbf{A1} & \textbf{A2} & \textbf{A3} & \textbf{B1} & \textbf{B2}\\ 
                                     
\toprule

QuickRecall\cite{jayakumar2014quickrecall}, Mementos\cite{ransford2012mementos} 
                            & Checkpt. & \xmark & \xmark & \xmark & \xmark & \cmark\\
                \rowcolor{gray!10}
DINO\cite{lucia2015DINO}, Ratchet\cite{woude2016ratchet}, Chinchilla\cite{maeng2018Chinchilla}     
                            & Checkpt & \cmark & \xmark & \xmark & \xmark & \cmark\\
Samoyed\cite{maeng2019Samoyed}
                            & Checkpt. & \cmark & \cmark &\xmark & \xmark & \cmark\\
\rowcolor{gray!10}                              
TICS\cite{kortbeek2020TICS}, CatNap\cite{maeng2020CatNap}
                            & Checkpt. &\cmark &\xmark &\cmark &\xmark &\cmark\\
Chain\cite{colin2016chain}, Alpaca\cite{alpaca}, Mayfly\cite{hester2017mayfly}, Coala\cite{majid2020Coala} Rehash~\cite{bakar2021rehash}
                            & Task-based &\cmark &\xmark&\xmark&\xmark &\xmark\\
 \rowcolor{gray!10} 
PureMEM\cite{durmaz2019puremem}
                            & Task-based & \cmark &\xmark &\xmark &\xmark & \cmark\\
Coati\cite{ruppel2019Coati}, InK\cite{yildirim2018ink}  
                            & Task-based & \cmark &\xmark & \cmark &\xmark &\xmark\\
%Hibernus\cite{balsamo2016hibernus++}, Harvos\cite{mottola2017harvos} 
%                           & Ch. & ? & ? & ? & ? & ?\\
                \rowcolor{yellow!30} 
{{\bf This Work} (\vmname/\langname) }
                            & Virtual Machine &\cmark &\cmark &\cmark &\cmark &\cmark\\
\bottomrule
\end{tabular}

\end{table}
